Supervision Exists Everywhere: A Data Efficient Contrastive Language-Image Pre-training Paradigm

Recently, large-scale Contrastive Language-Image Pre-training (CLIP) has attracted unprecedented attention for its impressive zero-shot recognition ability and excellent transferability to downstream tasks. However, CLIP is quite data-hungry and requires 400M image-text pairs for pre-training, thereby restricting its adoption. This work proposes a novel training paradigm, Data efficient CLIP (DeCLIP), to alleviate this limitation. We demonstrate that by carefully utilizing the widespread supervision among the image-text pairs, our De-CLIP can learn generic visual features more efficiently. Instead of using the single image-text contrastive supervision, we fully exploit data potential through the use of (1) self-supervision within each modality; (2) multi-view supervision across modalities; (3) nearest-neighbor supervision from other similar pairs. Benefiting from intrinsic supervision, our DeCLIP-ResNet50 can achieve 60.4% zero-shot top1 accuracy on ImageNet, which is 0.8% above the CLIP-ResNet50 while using 7.1 x fewer data. Our DeCLIP-ResNet50 outperforms its counterpart in 8 out of 11 visual datasets when transferred to downstream tasks. Moreover, Scaling up the model and computing also works well in our framework.Our code, dataset and models are released at: https://github.com/Sense-GVT/DeCLIP

==> DeCLIP/5_related_work/5_1_contrastive_learning.tex <==
% % \section{Related Work}
% \subsection{Contrastive Learning}
% Contrastive learning, as a pretext task of self-supervised training, has achieved remarkable success in visual representation learning. MoCo~\citep{he2020momentum} achieves comparative learning training by building a dynamic dictionary with a queue and a moving-averaged encoder. SimCLR~\citep{chen2020simple} selects the optimal data augmentation combination method, and adds a non-linear mapping after the encoder, discards the memory bank and adopts a larger batch size to calculate the contrastive learning loss. MoCo v2~\citep{chen2020improved} draws on the idea of SimCLR~\citep{chen2020simple} and improves on the basis of MoCo~\citep{he2020momentum}. SwAV~\citep{caron2020unsupervised} clusters various types of samples during training, and then distinguishes the clusters of each type, and proposes a new data augmentation method that mixes views of different resolutions.BYOL~\citep{grill2020bootstrap} adds the Predictor module to the Projector, and learns the mapping from online encoder to target encoder through Predictor. Only consider the positive sample pairs, and use the target network stop-gradient for training. SimSiam~\citep{chen2021exploring} removes the target encoder updated by momentum on the basis of BYOL~\citep{grill2020bootstrap}. Finding that stop-gradinent is the key to avoid training collapse. SEER~\citep{goyal2021self} and DnC~\citep{tian2021divide} discards the ImageNet~\citep{deng2009imagenet} dataset commonly used for training, and use a large amount of unlabeled data crawled from the network, so that the model can learn more general knowledge from a broader open data domain. In addition, with the popularity of vision transformer, MoCo v3~\citep{chen2021empirical} applies contrastive learning to the vision transformer network, and analyzes the characteristics of the vision transformer structure when training a contrastive learning model. DINO~\citep{caron2021emerging} designs an unlabeled self-supervised method with knowledge distillation by analyzing the characteristics of ViT~\citep{dosovitskiy2020image} features. In addition to the good effects, the learned features have a strong Interpretability. 

% In the field of NLP, in addition to common pretext tasks such as Mask Language Model~\citep{devlin2018bert}, there are gradually some ideas of self-supervised training sentence-embedding using contrast learning methods. BERT-CT~\citep{carlsson2021semantic} uses two models with the same structure and different parameters to generate two views for contrastive learning to obtain higher-quality sentence representation vectors.SimCSE~\citep{gao2021simcse} is trained by randomly dropout mask in the training phase, inputting the same sample into the same encoder twice, and obtaining two different representation vectors to construct contrastive learning sample pairs for training. ConSERT~\citep{yan2021consert} proposes a contrastivelearning framework based on contrastive learning and pre-training models, which includes three parts: data enhancement, BERT coding layer, and contrast loss layer, which improves the effect of pre-training models when transfer to downstream tasks. In general, recently, contrastive learning has made significant progress in the CV and NLP fields by constructing sample pairs for training programs.

==> DeCLIP/5_related_work/5_2_multimodal_learning.tex <==
\subsection{Multi-Modal Learning}
% Multi-modal learning has made significant progress on image-text tasks recent year, especially on large scale pre-training tasks, with amazing results.Their paradigm is mainly to use two encoders to respectively encode image and text information, and use contrastive learning for training. CLIP~\citep{radford2021learning} is a milestone work. It uses 400 million image-text data crawled on the Internet for training, and has achieved remarkable results in image-text retrieval task, zero-shot image recognition tasks and pre-training task. ALIGN~\citep{jia2021scaling} scales up the image-text data to 1 billion on the basis of CLIP~\citep{radford2021learning}. During training, the text encoder generates the “label” weights and uses a larger batchsize to achieve better results than CLIP~\citep{radford2021learning}.WenLan~\citep{huo2021wenlan} and EfficientCLIP~\citep{wang2021efficientclip} train Chinese pairs data. EfficientCLIP~\citep{wang2021efficientclip} uses Ensemble Confident Learning to make good use of single-modal text data during multi-modal training. With fewer training resources, it achieves the state-of-the-art performance on Chinese cross-modal retrieval tasks. CLIP2Video~\citep{fang2021clip2video} is based on the semantic space constructed by the CLIP~\citep{radford2021learning} model to capture motions at fine temporal video frames, re-align the tokens of video clips and phrases and enhance the multi-modal correlation to transfer the image-language pre-training model to video-text retrieval, achieve state-of-the-art performance on major text-to-video and video-to-text retrieval benchmarks.

% Although these works have achieved significant results on the basis of contrastive learning, because only the contrastive learning between image and text is carried out, the self-supervision of image and text  is ignored, so that when training large scale data, there is low data utilization. Therefore, we think more comprehensively about vision-language contrastive learning, and form a group contrastive learning  paradigm  composed of Image-Image contrastive learning, Text-Text contrastive learning, Image-Text contrastive learning, and Nearest-Neighbor-Text contrastive learning. 

==> DeCLIP/5_related_work/5_skeleton.tex <==
\paragraph{Pre-trained Models.} 

\paragraph{Supervisory Signals.}

\paragraph{Multi-modal Learning.}

==> DeCLIP/Statement/ethics_statement.tex <==
\section*{Ethics Statement}

==> DeCLIP/Statement/reproducibility_statement.tex <==
\section*{Reproducibility Statement}

==> DeCLIP/TODO.tex <==
% \paragraph{TODO(7.11-7.13)}

% \begin{itemize}
% \item Draw main workflow figure (SSL + Multi-View + NN).
% \item Finish first edition of introduction. Using 1-3 sentences to summarize the main concept of each paragraph. 
% \item Get the downstream baselines of CLIP (cls, det, seg).
% \item Train CLIP baseline on 30M/50M data (and evaluate on downstream tasks).
% \end{itemize}

% \paragraph{TODO(7.14-7.16)}

% \begin{itemize}
% \item Finish first edition of approach. 
% \item According to the intro/approach, write a clear experiments plan.
% \end{itemize}


% \paragraph{TODO(8.3-8.4)}

% \begin{itemize}
% \item Rewrite introduction.
% \item Run 28M CLIP experiments.
% \end{itemize}

% \paragraph{TODO(8.5-8.8)}

% \begin{itemize}
% \item Align the zero-shot validation in CLIP paper.
% \item Identify the effectiveness of SSL (SimSiam brings little improvement). 
% \item Fix downstream datasets \& get official CLIP's corresponding number.
% \item Grab more academic datasets, e.g. WIT.
% \item Write the first edition of approach.
% \end{itemize}


\paragraph{TODO(9.27)}

\begin{itemize}
    % \item Except for Language-Image in CLIP, we use image-text pairs. For any visual concepts, we use image. For any textual concepts, we use text.
    % \item How do you think the abstract? Our work IS an incremental work, such as roBERTa for BERT, DeiT for ViT, Deforamable DETR for DETR.
    \item Brain storm: Are there better names for self-supervision (SS), multi-view supervision (MVS), nearest neighbor supervision (NNS).
    % \item Exp in abstract: One sentence to show efficiency (R50/ViT). 2. One sentence to show downstream verification (9/10). 3. One sentence to show our work can scale up, no SOTA claim (RegNet-Y). Two reasons why we should put it up : 1. We actually have 2. Big tech companies might want to know, i.e. this result will convince them to use DeCLIP on their projects.
    \item \checkme{Whether the text encoder of CLIP scale up?}
    % \item \checkme{Our approach is double scaling up. Check the overall parameters of our RegNet-Y, CLIP R50x16 params.}
    \item \checkme{Check the config of CLIP R50x16.}
    % \item Redraw Fig.1, remove 3M experiments
    % \item Redraw Fig.2, maybe choose 10 out of 12? Refer GAIA paper(https://arxiv.org/pdf/2106.11346.pdf) for a good look. 
    % How to cheery pick? It is good if we can tell why we perform badly on these two datasets.
    \item Self-supervision for text. I think we need it to match (1) self-supervision within each modality;
    % \item \checkme{Fig.3 Not discriminative. Color deep. Text Language Modelling.}
    \item \checkme{Simsiam Text supervision}
    % \item Redraw Fig3 from detailed picture to skeleton?
    \item Scaling up models at Sec.3
    \item Ablation on Training Cost.
    \item Some visualization 1) attention map: our Declip can look more precisely at the object. 2) NN in dataset.
    % \item Format of tabel (Use ).
    % \item CLIP YFCC15M, our re-implementation.
    \item wikipedia query frequency top10w 
    \item \checkme{RegNetY-64GF: 276.237M/ResNetx64: 288M}
    \item \checkme{our work exceeds CLIP with releasing r50-ImageNet pretrain, exceeds some  CLIP CLIP with ViT-B/32-ImageNet21k pretrain, }
\end{itemize}

% \paragraph{TODO(9.30)}

% \begin{itemize}
%     \item For Fig.2, I look at the ImageNet results in the CLIP paper. It turns out that the performance of ImageNet pre-trained model is much lower than CLIP. If we draw it in Fig.2, Our gain might be not that significant. \lf{I suggest put the ImageNet performance at the table in experiments.}
    
    % \item Fig.2 need further improvements. Can we change 'DEC' to 'DeC'? How about the range of y-axis is either 4 (IN: 71-75, C100 68-72, PE 86-90, C10 87-91, SUN 70-74, AIR 46-50, DTD 74-78, Avg 77-81) or 6 (FL: 94-100, FO 81-87, CARS 77-83, CAL 89-95). The height of fig.2 should match that of fig.1 (shorter). We can also change the ratio of fig.1 and fig.2.
    
    

    % \item Best R50/ViT-B32 zero-shot. How to clarify our contribution to the community. \lf{Done: I put this part in last paragraph of intro.}
    
    % \item The introduction is somehow like related work, not a story. Rewrite it. \lf{Done: I re-wrote intro. once again on Sep.30. }
    % \end{itemize}

% \paragraph{TODO(10.1)}

% \begin{itemize}
    
    % \item According to fig.2 Our declip only outperforms clip in 8 out of 11 dataset (excluding average.) \lf{Done: Changing '9 in 11' to '8 in 11'. }
    
    % \item Rewrite related work. \lf{Done: I re-wrote related work on Oct.1. }
    
    % \item Fig.3 Not discriminative. Color deep. Text Language Modelling. \lf{Done: I re-drew Fig.3. }
    
    % \item We do not line up each components in the method part. Rewrite method. \lf{Half-way: I re-wrote till to Sec.3.2. Move Sec.3.3 to Oct.2. }
    
%     \item Original CLIP text encoder is not bidirectional, so how does the MLM (from bidirectional BERT) fit into this paradigm?
    
% \end{itemize}

\paragraph{TODO(10.2-3)} 
\begin{itemize}
    \item Rewrite Sec.3.3. \lf{Done: I re-worte Sec.3.3 on Oct.2.}
    
    \item The number in Fig.2 need to be a little bit larger.
    
    \item We should have CLIP-ImageNet results in Tab.3.
    
    \item Add image/text augmentations in Appendix.
    
    \item @lichen, I need you to fill the language SS in Sec 3.3.1.
    
    \item \checkme{A better order for Tab.4? It seems MVS brings most of the gain, how about SS - MVS - NNS?}
    
    \item Rewrite \& and reorganize exp and ablation study. \lf{Half-way to Sec4.1.}
    
    \item Put all the experiments, tables and figures in exp/ablation. Then I will rewrite them. 
    
    \item fig3. MLM \lf{Done: I added small circle above textual features to indidate MLL.}
    
    \item Appendix, more details about how to get the crawled data. Maybe provide some cost estimations.
    
    \item Missing: attention map of a image.
    
    \item Redraw Fig.9 x-axis should be time. It should have the declip curve as well. Suggest use the plot code of Fig.1
    
    \item Redraw Fig.6, how about 2 image-text pairs for CC/ YFCC/ Google? We could have some slight failure cases in this figure , we can explain it.
    
    \item double check eq.2
    
    \item Can we change order of SS and MVS?
    
    \item \checkme{Contribution, ablation on training cost, conclusion and appendix will be rewritten soon}
    
\end{itemize}




==> DeCLIP/back_up.tex <==
\paragraph{Original pre-training setup}

We train our \workname model from scratch on the collected 88M dataset, which image encoder are ResNet50 modified from CLIP~\citep{radford2021learning} and ViT-B/32~\citep{dosovitskiy2020image}, text encoder is a 12-layer transformer structure from CLIP~\citep{radford2021learning}, with the context length 77, the transformer width 512, and the transformer heads 8.  Both text projection and visual projection dimensions are 1024. Image SS uses SimSiam~\citep{chen2021exploring} method, prediction module is a 2-layer MLP, which hidden dimensions is 512 and output dimensions is 1024, projection module  is a 3-layer MLP, which hidden and output dimensions are both 1024. Text SS uses the Masked Language Model~\citep{devlin2018bert} to select 15\% of all words in the corpus for random mask as the pretext task. In MVS, image encoder uses augmentation from MoCo v2~\citep{chen2020improved} and text encoder uses EDA~\citep{wei2019eda} as augmentation, NNS is text nearest neighbor specifically finding an additional text supervision for each text by calculating the similarity of the text in a mini-batch. 
% In addition, loss weight of ${\alpha}$, ${\beta}$ and ${\gamma}$ are all 0.2. During training, ResNet-50 and ViT-B/32 both use the resolution of $224\times224$ pixels, and the text transformer uses input size with a maximum context length of 77. The learnable temperature parameter $\tau$ was initialized to the equivalent of 0.07. 
% ResNet-50 uses the FP16-SGD optimizer and batch size 10,240  for training, with an initial learning rate of 0.01, warmed up linearly to 0.2 in one epoch steps, which weight decay is 0.0001 and momentum is 0.9.
% When training ViT-B/32, we use FP16-AdamW-SGD with batch size 20,480 for stable training. In detail, When training the text encoder, we use the SGD optimizer which learning rate warmed up linearly from 1e-3 to 0.02, the weight decay rate is set as 1e-4 and the momentum is set as 0.9. For the image encoder, we use AdamW optimizer which learning rate warmed up linearly from 1e-4 to 1e-3, and the weight decay rate is set as 0.05.
% ViT-B/32 model uses FP16-AdamW-SGD and batchsize 20480 for training. For the stability of training, the text encode uses SGD optimizer which learning rate warmed up linearly to 0.02 from 1e-3 in one epoch, weight decay is 1e-4 and momentum is 0.9. The image encode uses AdamW optimizer which learning rate warmed up linearly to 1e-3 from 1e-4 in one epoch, and weight decay is set as 0.05.
Both ResNet-50 and ViT-B/32 use Cosine learning rate decay to train 32 epochs. 
ResNet-50 requires 80 V100 GPUs for training for 8 days, and ViT-B/32 requires 80 V100 GPUs for training for 10 days. When scaling up models, we use RegNetY-64GF~\citep{2020Designing,goyal2021self} as image encoder and BERT~\citep{devlin2018bert} as text encoder, training 32 epochs with batch size 20,480, which requires 160 V100 GPUs for training for 21 days.




% \workname's pre-training ability by linear classification on frozen features: the pretrained image encoder is fixed and used to extract features. 
Firstly, the features of each image are extracted from the pretrained image encoder and form a full-batch. 
Both train and eval resolution are $224\times224$ with frozen visual features.
% Secondly, we train a fc-based classifier using pytorch’s L-BFGS implementation with maximum 1,000 full-batch iterations.
Secondly, we train a fc-based classifier by the L-BFGS optimizer with 1,000 full-batch iterations.
% full-batch 
% To conduct fair comparison with
Finally, we determine the L2 regularization strength using a hyperparameter $\lambda$ sweep on the validation sets over the range between 1e-6 and 1e6 with 16 logarithmically spaced steps.
% For each dataset, the 
% To conduct fair comparison, the metric and division for each dataset is consistent with that of clip~\citep{radford2021learning}.
% The individual linear probe scores are provided in Table \ref{tab:downstream datasets}.





After pre-training, we use natural language to refer to visual concepts enabling the zero-shot ability of our model.
As shown in Fig.~\ref{fig:IN_zero_shot}, when using 15M pairs, our \workname-ResNet50 is 10.6\% higher than the number reported in ~\citet{radford2021learning}. 
More data leads to better accuracy. 
When the data amount reaches 56M (29M open-source + 27M web-crawled), our model can achieve 60.4\% accuracy, 0.8\% above the CLIP-ResNet50, while using 7.1$\times$ fewer data. 
As described in Tab.~\ref{tab:zero-shot result}, with our full data, our best ResNet50/ViT-B32 models boost the zero-shot performance to 62.5\% and 66.2\%, nearly 3.0\% higher than the best number reported for these two architectures. Moreover, our \workname-ResNet50 is even 0.3\% better than CLIP-ResNet101, revealing the effectiveness and efficiency of our framework. Scaling up model capacity works in our framework as well. Our biggest \workname-RegNetY-64GF achieves \checkme{73.7\%} accuracy, which is 0.1\% above CLIP ResNet50$\times$64 with fewer parameters. 



\begin{table*}[t]
\caption{\label{tab:zero-shot result} Zero-shot top1 performance of \workname on ImageNet dataset. \checkme{We might need model parameters here. We can also put CLIP-ViT-Lx14 on it.} }
\label{sample-table}
\begin{center}
\begin{footnotesize}
\begin{sc}
\begin{tabular}{cccccc}
   \toprule  
   %\multicolumn{5}{r}{}  \\
   \textbf{Model}         & \textbf{Backbone} & \textbf{Parameters}  & \textbf{Data Size}   &\textbf{Batch Size}  & \textbf{Zero-Shot} \\
   \midrule   
   CLIP         &ResNet50 &24M &400M & 32,768 &59.6	\\
%   \textbf{DeCLIP}       &\textbf{ResNet50} &24M &\textbf{56M}  & \textbf{10,240} &\textbf{60.4(+0.8)} 	\\
   DeCLIP       &ResNet50 & \textbf{24M} &\textbf{88M($\downarrow$ 4.5$\times$)}  & \textbf{10,240} &\textbf{62.5($\uparrow$  +2.9)} 	\\
      CLIP         &ResNet101 &42M &400M & 32,768 &62.2	\\

   \midrule
   CLIP         &ViT-B/32 &88M &400M & 32,768 &63.2	\\
   DeCLIP       &ViT-B/32 &\textbf{88M} &\textbf{88M($\downarrow$ 4.5$\times$)}   & \textbf{20,480} &\textbf{66.2($\uparrow$ +3.0)}	\\
  \midrule
  CLIP         &ResNet50$\times$64 &291M  &400M & 32,768 &73.6	\\
  DeCLIP       &RegNetY-64GF &\textbf{276M} &\textbf{88M($\downarrow$ 4.5$\times$)}   & \textbf{20,480} &\textbf{73.7($\uparrow$ +0.1)}	\\
  \bottomrule
\end{tabular}
\end{sc}
\end{footnotesize}
\end{center}
\end{table*}



\begin{table*}[h]
\caption{\label{tab:downstream result} Linear probe performance on various pre-trained models over 11 datasets.}
\label{sample-table}
\begin{center}
\begin{scriptsize}
\begin{sc}
\begin{tabular}{cccccccccccccc}
\toprule
%\rotatebox{90}{Model} & \rotatebox{90}{Backbone}  & \rotatebox{90}{CIFAR10} & \rotatebox{90}{CIFAR100} & \rotatebox{90}{Food101} & \rotatebox{90}{Pets} & \rotatebox{90}{Fowers} & \rotatebox{90}{SUN397} & \rotatebox{90}{Cars} & \rotatebox{90}{DTD} & \rotatebox{90}{Caltech} & \rotatebox{90}{Aircraft} & \rotatebox{90}{ImageNet}    \\
\textbf{Model} & \textbf{Backbone}  &\textbf{\rot{Pets}} & \textbf{\rot{CIFAR10}} & \textbf{\rot{CIFAR100}}  & \textbf{\rot{SUN}} & \textbf{\rot{Food101}} &\textbf{\rot{Flowers}}       \\
\midrule\textbf{}
%ResNet &ResNet50     & 92.4 & 91.8 & 74.5 & 60.5 & 71.3  & 90.8 \\
CLIP &ResNet50     & 88.2 & 88.7 & 70.3 & 73.3 & 86.4  & 96.1 \\
De-CLIP &ResNet50   & \textbf{88.7} &\textbf{89.8} & \textbf{71.2 }& 72.8 & 82.7  & \textbf{99.2}  \\
\midrule
CLIP &ViT-B/32              & 90.0  & 95.1 & 80.5 & 76.6 & 88.8 & 96.9   \\
DeCLIP &ViT-B/32            & 89.2  & \textbf{96.5} & \textbf{84.7 }& 75.0 & 85.0 & \textbf{99.1} \\
% \bottomrule


\toprule
%\rotatebox{90}{Model} & \rotatebox{90}{Backbone}  & \rotatebox{90}{CIFAR10} & \rotatebox{90}{CIFAR100} & \rotatebox{90}{Food101} & \rotatebox{90}{Pets} & \rotatebox{90}{Fowers} & \rotatebox{90}{SUN397} & \rotatebox{90}{Cars} & \rotatebox{90}{DTD} & \rotatebox{90}{Caltech} & \rotatebox{90}{Aircraft} & \rotatebox{90}{ImageNet}    \\
\textbf{Model} & \textbf{Backbone}  & \textbf{Cars}  & \textbf{Caltech} & \textbf{Aircraft} &\textbf{DTD} & \textbf{ImageNet} & \textbf{Average}    \\
\midrule

CLIP &ResNet50       & 78.3  & 89.6 & 49.1 & 76.4 &73.3 &79.1\\
De-CLIP &ResNet50   & \textbf{81.7} & \textbf{93.9} & 48.4 & \textbf{76.8 }&\textbf{74.0} &\textbf{79.9(+0.8)} \\
\midrule
CLIP &ViT-B/32               & 81.8 & 93.0 & 52.0 & 76.5 & 76.1 & \textbf{82.5}\\
DeCLIP &ViT-B/32             & 81.6 & \textbf{94.8 }& \textbf{53.5} & \textbf{78.5} & 75.3 &\textbf{83.0 (+0.5)}\\
\bottomrule


\end{tabular}
\end{sc}
\end{scriptsize}
\end{center}
\end{table*}


==> DeCLIP/backup/title_candidate.tex <==
\section{Title candidate}
\subsection{DECLIP: Data-Efficient Contrastive Language-Image Pre-training via Data Exhaustion}
\subsection{DECLIP: Data-Efficient Language-Supervised Zero-Shot Learning via Data Exhaustion}
\subsection{E-CLIP: An Efficient Language-Supervised Zero-Shot Learning Paradigm via Data Exhaustion}
\subsection{Exhausting Your Data: An Efficient Language-Supervised Zero-Shot Learning Paradigm}
\subsection{Exhausting Every Supervision of Your Multi-Modal Data}
\subsection{Supervision Exists Everywhere in Your Multi-Modal Data}
\subsection{Supervision Exists Everywhere: An Efficient Language-Supervised Zero-Shot Learning Paradigm}
\subsection{Supervision Exists Everywhere: An Efficient Contrastive Language-Image Pre-training Paradigm}
\subsection{Synonym: exhausting, draining, depleting}

==> DeCLIP/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> pseudocode.tex <==

% \documentclass[11pt]{article}
% \usepackage{CJK}
% \usepackage[top=2cm, bottom=2cm, left=2cm, right=2cm]{geometry}
% \usepackage{amsmath}
% \usepackage{indentfirst}

% \floatname{algorithm}{算法}
% \renewcommand{\algorithmicrequire}{\textbf{输入:}}
% \renewcommand{\algorithmicensure}{\textbf{输出:}}

% TODO Repaint the pseudo code
\begin{algorithm}
    \caption{DeCLIP}
    \begin{algorithmic}[1] %每行显示行号
        \Require $I$, $\tilde{I}$, $T$, $\tilde{T}$, $image\_encoder$, $text\_encoder$, $Feature\_Queue$
        % \Ensure $Logits$
        \Function {Batch-Updating}{$I$, $\tilde{I}$, $T$, $\tilde{T}$}
            \State \textcolor[RGB]{64,128,128}{$\#$ Get The Features of The Current Batch.}
            % \State $I_f \gets image\_encoder(I)$
            % \State $\tilde{I}_f \gets image\_encoder(\tilde{I})$
            % \State $T_f \gets text\_encoder(T)$
            % \State $\tilde{T}_f \gets text\_encoder(\tilde{T})$
            \State $I_f, \tilde{I}_f \gets image\_encoder(I), image\_encoder(\tilde{I})$
            \State $T_f, \tilde{T}_f \gets text\_encoder(T), text\_encoder(\tilde{T})$
            \State $T_{NN} \gets$ \Call{Nearest-Neighbor}{$Feature\_Queue, T_f$}
            \State
            \State \textcolor[RGB]{64,128,128}{$\#$ Calculate The losses.}
            \State $L_{CLIP} \gets$ \Call{InfoNCE-Loss}{$I_f, T_f$}
            \State $L_{SS} \gets$ \Call{Image-SS-Loss}{$I_f, \tilde{I}_f$} + \Call{Text-SS-Loss}{$T_f$}
            \State $L_{MVS} \gets$ \Call{InfoNCE-Loss}{$I_f, \tilde{T}_f$} + \Call{InfoNCE-Loss}{$\tilde{I}_f, T_f$} + \Call{InfoNCE-Loss}{$\tilde{I}_f, \tilde{T}_f$}
            \State $L_{NNS} \gets$ \Call{InfoNCE-Loss}{$\tilde{I}_f, \tilde{T}_{NN}$}
            \State $L_{\workname} \gets (1 - \alpha - \beta - \gamma)L_{CLIP} + \alpha L_{SS} + \beta L_{MVS} + \gamma L_{NNS}$
            \State
            \State \textcolor[RGB]{64,128,128}{$\#$ Update The Network.}
            % \State \Call{Update-NetWork}{$image\_encoder, L_{\workname}$}
            % \State \Call{Update-NetWork}{$text\_encoder, L_{\workname}$}
            % \State $Feature\_Queue \gets$ \Call{Update-FeatureQueue}{$Feature\_Queue, T_f$}
            \State $image\_encoder \gets$ \Call{Backward-Update}{$image\_encoder, L_{\workname}$}
            \State $text\_encoder \gets$ \Call{Backward-Update}{$text\_encoder, L_{\workname}$}
            \State $Feature\_Queue \gets$ \Call{FIFO-Update}{$Feature\_Queue, T_f$}
        \EndFunction
        \State
        \Function {Image-SS-Loss}{$I_f, \tilde{I}_f$}
            \State $z, \tilde{z} \gets image\_encoder.proj(I_f), image\_encoder.proj(\tilde{I}_f)$
            \State $p, \tilde{p} \gets image\_encoder.pred(z), image\_encoder.pred(\tilde{z})$
            \State $z, \tilde{z} \gets z.detach(), \tilde{z}.detach()$
            \State \textcolor[RGB]{64,128,128}{$\#$ Calculate the Negative Cosine Similarity loss.}
            \State $L_{Image-SS} \gets NCS(p, \tilde{z}) / 2 + NCS(\tilde{p}, z) / 2$  
            \State \Return{$L_{Image-SS}$}
        \EndFunction
        \State
        \Function {Text-SS-Loss}{$T_f$}
            \State \textcolor[RGB]{64,128,128}{$\#$ Get The Masking GT when performing the text-encoder.}
            \State $W_f, W_{gt} \gets T_f.word\_feat, T_f.mask\_id$
            % \textcolor{gray}{$\#$ $W_f$ and $W_{gt}$ represents the features and masked words, respectively.}
            \State $W_{pred} \gets text\_encoder.pred(W_f)$
            \State \textcolor[RGB]{64,128,128}{$\#$ Calculate the Cross-Entropy loss.}
            \State $L_{Text-SS} \gets CE(W_{gt}, W_{pred})$  
            \State \Return{$L_{Text-SS}$}
        \EndFunction
        
    \end{algorithmic}
\end{algorithm}

